Labelled calculi for lattice-based modal logics

We introduce labelled sequent calculi for the basic normal non-distributive modal logic L and 31 of its axiomatic extensions, where the labels are atomic formulas of a first order language which is interpreted on the canonical extensions of the algebras in the variety corresponding to the logic L. Modular proofs are presented that these calculi are all sound, complete and conservative w.r.t. L, and enjoy cut elimination and the subformula property. The introduction of these calculi showcases a general methodology for introducing labelled calculi for the class of LE-logics and their analytic axiomatic extensions in a principled and uniform way.

==> CanonicalSequents.tex <==
\section{Canonical sequents, display property, and distributivity}

We recall that in the general non distributive case $\mathbf{A.L}\Sigma$, Lemma
\ref{lem:exacttwo} guarantees that if a nominal (resp.~conominal) occurs in a derivable sequent $s$, then it occurs exactly twice.

%where the first occurrence is in precedent position and the second occurrence is in succedent position. Moreover, derivable $\mathbf{A.L}\Sigma$-sequents $\Gamma \vdsah \Delta$ are single-conclusion, namely $\Delta = \sigma$ for some well-formed structure $\sigma$.

The following statement further specifies the shape of derivable sequents. 

\begin{proposition}[Single-conclusion sequents and labelled formulas]
\label{thm:SingleConclusion}
For derivable $\mathbf{A.L}\Sigma$-sequent $s = \Gamma \vdash \Delta$, $\Delta = \sigma$ for some well-formed structure $\sigma$ (i.e.~$s$ is single-conclusion), and $s$ contains exactly two labelled formulas, one in precedent position and the other in succedent position.
\textcolor{red}{ADD: in general case, $s$ contains $n \in \{2,\ldots,m\}$ labelled formulae, where $m$ is the number of leaves in the skeleton portion of the syntax tree.}
\end{proposition}

\begin{proof}
The proof is by induction on the height of derivations.
\end{proof}

The proof of Lemma \ref{lem:exacttwo} relies on the side condition required for the conclusions of switch rules (except for S$\cnomm$ and S$\nomj$), namely that nominals or conominals occurring in the nonparametric structures in the conclusion  must be fresh. Lemma \ref{lem:exacttwo} is used in Appendix \ref{ALIsAProperLabelledCalculus} for showing that $\mathbf{A.L}\Sigma$ enjoys the display property (see Proposition \ref{thm:DisplayPropertyAL}). In this section, we provide an alternative proof of the display property using the notion of {\em canonical sequent} (see Definition \ref{def:CanonicalSequents} and Lemma \ref{thm:CanonicalForm} below). Notice that neither Lemma \ref{lem:exacttwo} nor Proposition \ref{thm:SingleConclusion} is used in the proof of Lemma \ref{thm:CanonicalForm}, therefore the side condition imposed on the conclusion of switch rules can be dropped (while we still retain the side condition imposed on the premises of switch rules, namely that nominals or conominals occurring in the nonparametric structures in the premise must be fresh). \textcolor{red}{ADD: notice that Lemma 1 still holds without the strict side condition of the switch rule if we start bottom up from formulae without structural connectives.}

\subsection{Preliminary observations on cut elimination and policies on the choice of nominals/conominals}

First, we fix the notation.

\begin{remark}[Notation]
\label{rem:TermVariableOrdering}
We use $\cnomm_0, \cnomm_2, \cnomm_4, \ldots$ and $\nomj_1, \nomj_3, \nomj_5, \ldots$, namely we use even numbers for conominals term variables and odd numbers for nominal term variables. Moreover, we consider the orderings of term variables induced by the subscripts, i.e.~$\cnomm_0 < \cnomm_2 < \cnomm_4$ and $\nomj_1 < \nomj_3 < \nomj_5 < \ldots$. Finally, if a structure $x \leq y$ occurs in $\Delta$ in a sequent $\Gamma \vdash \Delta$, we write $y \geq x$.
\end{remark}

We now recall the {\em side conditions of switch rules} (see Section \ref{sec:LabelledCalculusAL}):
\begin{itemize}
\item (a) the nominals/conominals occurring in the nonparametric structures in the {\em conclusion} of $S$ are fresh (except for S$\cnomm$ and S$\nomj$);
\item (b) the nominals/conominals occurring in the nonparametric structures in the {\em premise} of $S$ are fresh.
\end{itemize}

In this section, we will consider the following policies for choosing nominals or conominals in a derivation. We use the expression {\em nominal or conominal with the smallest compatible subscripts}, where ``smallest'' means the smallest w.r.t.~the ordering of term variables (see Remark \ref{rem:TermVariableOrdering}) and ``compatible'' means that the choice still preserve the side conditions of rules (in particular, of switch rules as defined in Section \ref{sec:LabelledCalculusAL}) and the well-formedness of structures (see the side condition in the definition of the language in Section \ref{sec:LabelledCalculusAL}).

\begin{itemize}
\item {\em (1) Policy on the choice of nominals/conominals.} Proceeding top-down, switch rules always pick the nominal or conominal with the smallest compatible subscript (i.e.~they pick the very same nominal or conominal in each history-tree of the congruent structures, namely the nominal or conominal introduced by an initial rule, $\wbox_P$, or $\wdia_S$), while $\wbox_P, \wdia_S, C, 4$ pick pick nominal or conominal with increasing subscripts (i.e.~they pick fresh nominals or conominals in the branch). 
\item {\em (2) Policy on the choice of nominals/conominals.} Proceeding top-down, switch rules always pick nominals or conominals with increasing subscripts (i.e.~they pick fresh nominals or conominals in the branch), while $\wbox_P, \wdia_S, C, 4$ pick the nominal or conominal with the smallest compatible subscript (i.e.~they pick the very same nominal or conominal in each history-tree of congruent structures). 
\end{itemize}

In the rest of the section, we emphasize in red the history-tree of cut formulas in derivations to facilitate the tracking of nominals/conominals occurring in congruent structures.

In the following derivation $\pi_1$ we use initial rules with empty contexts and non-invertible logical rules $\aand_P, \aor_S, \wbox_P, \wdia_S$ (in what follows whenever we say ``non-invertible logical rules'' we refer to this list of rules).  

Notice that Policy (1) generates a correct $\mathbf{A.L}\Sigma$-derivation $\pi_1$. In particular, every application of a switch rule $S$ in $\pi_1$ respects the side conditions of switch rules $S$ (on the conclusions and on the premises of $S$).

Proceeding top-down, Policy (1) preserves the subscripts occurring in the approximants of principal formulas (e.g.~in $\pi_1$ if two congruent occurrences of $\wbox A$ are approximated by nominals $\nomj_k$ and $\nomj_\ell$, then $k = \ell$). Therefore, in the parametric stage of the cut elimination procedure, the newly generated cuts are well-defined and there is no need to rename the nominals or conominals of the original derivation. Below we produce $\pi_1$ and $\pi_1'$, where $\pi_1'$ is generated as a proof transformation of $\pi_1$ in the parametric cut elimination step.

{\small
\begin{center}
\begin{tabular}{c}
$\pi_1$: Policy (1) \\
both cut formulas are parametric \\
\hline
\rule[0mm]{0mm}{23mm}
\AXC{$\pi_{1.1}$}
\RL{\fns Id$_{\,A\leq\cnomm_0}$}
\UIC{$A \leq \cnomm_0 \vd \cnomm_0 \geq A$}
\LL{\fns $\wbox_P$}
\UIC{$\nomj_1 \leq \wbox A, A \leq \cnomm_0 \vd \wbox \cnomm_0 \geq \nomj_1$}
\RL{\fns $\wbox_S$}
\UIC{$\nomj_1 \leq \wbox A \vd \textcolor{red}{\wbox A \geq \nomj_1}$}
\RL{\fns S}
\UIC{$\textcolor{red}{\wbox A \leq \cnomm_0} \vd \cnomm_0 \geq \wbox A$}
\LL{\fns $\wbox_P$}
\UIC{$\nomj_3 \leq \wbox \wbox A, \textcolor{red}{\wbox A \leq \cnomm_0} \vd \wbox \cnomm_0 \geq \nomj_3$}
\RL{\fns $\bdia \dashv \wbox$}
\UIC{$\nomj_3 \leq \wbox \wbox A, \textcolor{red}{\wbox A \leq \cnomm_0} \vd \cnomm_0 \geq \bdia \nomj_3$}
\RL{\fns S}
\UIC{$\nomj_1 \leq \bdia \nomj_3, \nomj_3 \leq \wbox \wbox A \vd \textcolor{red}{\wbox A \geq \nomj_1} $}
%
\AXC{$\pi_{1.2}$}
\RL{\fns Id$_{\,A\leq\cnomm_0}$}
\UIC{$A \leq \cnomm_0 \vd \cnomm_0 \geq A$}
\LL{\fns $\wbox_L$}
\UIC{$\textcolor{red}{\nomj_1 \leq \wbox A}, A \leq \cnomm_0 \vd \wbox \cnomm_0 \geq \nomj_1$}
\RL{\fns $\bdia \dashv \wbox$}
\UIC{$\textcolor{red}{\nomj_1 \leq \wbox A}, A \leq \cnomm_0 \vd \cnomm_0 \geq \bdia \nomj_1$}
\RL{\fns S}
\UIC{$\nomj_3 \leq \bdia \nomj_1, \textcolor{red}{\nomj_1 \leq \wbox A} \vd A \geq \nomj_3$}
\RL{\fns $\wdia_R$}
\UIC{$\nomj_3 \leq \bdia \nomj_1, \textcolor{red}{\nomj_1 \leq \wbox A}, \wdia A \leq \cnomm_2 \vd \cnomm_2 \geq \wdia \nomj_3$}
\LL{\fns $\wdia \dashv \bbox$}
\UIC{$\nomj_3 \leq \bdia \nomj_1, \textcolor{red}{\nomj_1 \leq \wbox A}, \wdia A \leq \cnomm_2 \vd \bbox \cnomm_2 \geq \nomj_3$}
\RL{\fns S}
\UIC{$\textcolor{red}{\nomj_1 \leq \wbox A}, \wdia A \leq \cnomm_2, \bbox \cnomm_2 \leq \cnomm_0 \vd \cnomm_0 \geq \bdia \nomj_1$}
\LL{\fns $\bdia \dashv \wbox^{-1}$}
\UIC{$\textcolor{red}{\nomj_1 \leq \wbox A}, \wdia A \leq \cnomm_2, \bbox \cnomm_2 \leq \cnomm_0 \vd \wbox \cnomm_0 \geq \nomj_1$}
%
\RL{\fns Cut$_{\,\nomj_1 \leq \wbox A}$}
\BIC{$\nomj_1 \leq \bdia \nomj_3, \nomj_3 \leq \wbox \wbox A, \wdia A \leq \cnomm_2, \bbox \cnomm_2 \leq \cnomm_0 \vd \wbox \cnomm_0 \geq \nomj_1$}
\DP
 \\
\end{tabular}
\end{center}
}

{\small
\begin{center}
\begin{tabular}{c}
\rotatebox[origin=c]{-90}{$\rightsquigarrow$} \rule[-2mm]{0mm}{6mm}\\
$\pi_1'$: Policy (1) where no renaming of term variables is needed \\
exactly one cut formula is principal \\
\hline
\rule[0mm]{0mm}{32mm}
\AXC{$\pi_{1.1}$}
\RL{\fns Id$_{\,A \leq \cnomm_0}$}
\UIC{$A \leq \cnomm_0 \vd \cnomm_0 \geq A$}
\LL{\fns $\wbox_P$}
\UIC{$\nomj_1 \leq \wbox A, A \leq \cnomm_0 \vd \wbox \cnomm_0 \geq \nomj_1$}
\RL{\fns $\wbox_S$}
\UIC{$\nomj_1 \leq \wbox A \vd \textcolor{red}{\wbox A \geq \nomj_1}$}
%
\AXC{$\pi_{1.2}$}
\RL{\fns Id$_{\,A\leq\cnomm_0}$}
\UIC{$A \leq \cnomm_0 \vd \cnomm_0 \geq A$}
\LL{\fns $\wbox_L$}
\UIC{$\textcolor{red}{\nomj_1 \leq \wbox A}, A \leq \cnomm_0 \vd \wbox \cnomm_0 \geq \nomj_1$}
\RL{\fns $\bdia \dashv \wbox$}
\UIC{$\textcolor{red}{\nomj_1 \leq \wbox A}, A \leq \cnomm_0 \vd \cnomm_0 \geq \bdia \nomj_1$}
\RL{\fns S}
\UIC{$\nomj_3 \leq \bdia \nomj_1, \textcolor{red}{\nomj_1 \leq \wbox A} \vd A \geq \nomj_3$}
\RL{\fns $\wdia_R$}
\UIC{$\nomj_3 \leq \bdia \nomj_1, \textcolor{red}{\nomj_1 \leq \wbox A}, \wdia A \leq \cnomm_2 \vd \cnomm_2 \geq \wdia \nomj_3$}
\LL{\fns $\wdia \dashv \bbox$}
\UIC{$\nomj_3 \leq \bdia \nomj_1, \textcolor{red}{\nomj_1 \leq \wbox A}, \wdia A \leq \cnomm_2 \vd \bbox \cnomm_2 \geq \nomj_3$}
\RL{\fns S}
\UIC{$\textcolor{red}{\nomj_1 \leq \wbox A}, \wdia A \leq \cnomm_2, \bbox \cnomm_2 \leq \cnomm_0 \vd \cnomm_0 \geq \bdia \nomj_1$}
\LL{\fns $\bdia \dashv \wbox^{-1}$}
\UIC{$\textcolor{red}{\nomj_1 \leq \wbox A}, \wdia A \leq \cnomm_2, \bbox \cnomm_2 \leq \cnomm_0 \vd \wbox \cnomm_0 \geq \nomj_1$}
%
\RL{\fns Cut$_{\,\nomj_1 \leq \wbox A}$}
\BIC{$\nomj_1 \leq \wbox A, \wdia A \leq \cnomm_2, \bbox \cnomm_2 \leq \cnomm_0 \vd \wbox \cnomm_0 \geq \nomj_1$}
\RL{\fns S}
\UIC{$\wdia A \leq \cnomm_2, \bbox \cnomm_2 \leq \cnomm_0, \wbox \cnomm_0 \leq \cnomm_4 \vd \cnomm_4 \geq \wbox A$}
\LL{\fns $\wbox_P$}
\UIC{$\nomj_3 \leq \wbox \wbox A, \wdia A \leq \cnomm_2, \bbox \cnomm_2 \leq \cnomm_0, \wbox \cnomm_0 \leq \cnomm_4 \vd \wbox \cnomm_4 \geq \nomj_3$}
\RL{\fns $\bdia \dashv \wbox$}
\UIC{$\nomj_3 \leq \wbox \wbox A, \wdia A \leq \cnomm_2, \bbox \cnomm_2 \leq \cnomm_0, \wbox \cnomm_0 \leq \cnomm_4 \vd \cnomm_4 \geq \bdia \nomj_3$}
\RL{\fns S}
\UIC{$\nomj_1 \leq \bdia \nomj_3, \nomj_3 \leq \wbox \wbox A, \wdia A \leq \cnomm_2, \bbox \cnomm_2 \leq \cnomm_0 \vd \wbox \cnomm_0 \geq \nomj_1$}
\DP
 \\
\end{tabular}
\end{center}
}

We now provide a new derivation $\pi_2 \equiv \pi_1$ where initial rules with empty contexts and non-invertible logical rules are used as well, but implementing a dual policy on the choice of nominal and conominal.

Notice that Policy (2) generates a correct $\mathbf{A.L}\Sigma$-derivation $\pi_2$. In particular, every application of a switch rule $S$ in $\pi_2$ respects the side conditions of switch rule $S$ (on the conclusions and on the premises of $S$).

Proceeding top-down, Policy (2) increases the subscripts occurring in the approximants of congruent formulas (e.g.~in $\pi_2$ if two congruent occurrences of $\wbox A$ are approximated by nominals $\nomj_k$ and $\nomj_\ell$, then $k < \ell$). Therefore, in the parametric stage of the cut elimination procedure, the newly generated cuts are not well-defined and there is the need to rename nominals or conominals of the original derivation in exactly one of the proof sections immediately above the premises of the original cut.\footnote{We need to show that after the renaming we still have a correct proof section.} Below we produce $\pi_2$ and $\pi_2'$, where $\pi_2'$ is generated as a proof transformation of $\pi_2$ in the parametric cut elimination step.

{\small
\begin{center}
\begin{tabular}{c}
$\pi_2$: Policy (2) \\
both cut formulas are parametric \\
\hline
\rule[0mm]{0mm}{23mm}
\AXC{$\pi_{2.1}$}
\RL{\fns Id$_{\,A\leq\cnomm_0}$}
\UIC{$A \leq \cnomm_0 \vd \cnomm_0 \geq A$}
\LL{\fns $\wbox_P$}
\UIC{$\nomj_1 \leq \wbox A, A \leq \cnomm_0 \vd \wbox \cnomm_0 \geq \nomj_1$}
\RL{\fns $\wbox_S$}
\UIC{$\nomj_1 \leq \wbox A \vd \textcolor{red}{\wbox A \geq \nomj_1}$}
\RL{\fns S}
\UIC{$\textcolor{red}{\wbox A \leq \cnomm_2} \vd \cnomm_2 \geq \wbox A$}
\LL{\fns $\wbox_P$}
\UIC{$\nomj_1 \leq \wbox \wbox A, \textcolor{red}{\wbox A \leq \cnomm_2} \vd \wbox \cnomm_2 \geq \nomj_1$}
\RL{\fns $\bdia \dashv \wbox$}
\UIC{$\nomj_1 \leq \wbox \wbox A, \textcolor{red}{\wbox A \leq \cnomm_2} \vd \cnomm_2 \geq \bdia \nomj_1$}
\RL{\fns S}
\UIC{$\nomj_3 \leq \bdia \nomj_1, \nomj_1 \leq \wbox \wbox A \vd \textcolor{red}{\wbox A \geq \nomj_3} $}
%
\AXC{$\pi_{2.2}$}
\RL{\fns Id$_{\,A\leq\cnomm_0}$}
\UIC{$A \leq \cnomm_0 \vd \cnomm_0 \geq A$}
\LL{\fns $\wbox_L$}
\UIC{$\textcolor{red}{\nomj_3 \leq \wbox A}, A \leq \cnomm_0 \vd \wbox \cnomm_0 \geq \nomj_3$}
\RL{\fns $\bdia \dashv \wbox$}
\UIC{$\textcolor{red}{\nomj_3 \leq \wbox A}, A \leq \cnomm_0 \vd \cnomm_0 \geq \bdia \nomj_3$}
\RL{\fns S}
\UIC{$\nomj_5 \leq \bdia \nomj_3, \textcolor{red}{\nomj_3 \leq \wbox A} \vd A \geq \nomj_5$}
\RL{\fns $\wdia_R$}
\UIC{$\nomj_5 \leq \bdia \nomj_3, \textcolor{red}{\nomj_3 \leq \wbox A}, \wdia A \leq \cnomm_0 \vd \cnomm_0 \geq \wdia \nomj_5$}
\LL{\fns $\wdia \dashv \bbox$}
\UIC{$\nomj_5 \leq \bdia \nomj_3, \textcolor{red}{\nomj_3 \leq \wbox A}, \wdia A \leq \cnomm_0 \vd \bbox \cnomm_0 \geq \nomj_5$}
\RL{\fns S}
\UIC{$\textcolor{red}{\nomj_3 \leq \wbox A}, \wdia A \leq \cnomm_0, \bbox \cnomm_0 \leq \cnomm_2 \vd \cnomm_2 \geq \bdia \nomj_3$}
\LL{\fns $\bdia \dashv \wbox^{-1}$}
\UIC{$\textcolor{red}{\nomj_3 \leq \wbox A}, \wdia A \leq \cnomm_0, \bbox \cnomm_0 \leq \cnomm_2 \vd \wbox \cnomm_2 \geq \nomj_3$}
%
\RL{\fns Cut$_{\,\nomj_3 \leq \wbox A}$}
\BIC{$\nomj_3 \leq \bdia \nomj_1, \nomj_1 \leq \wbox \wbox A, \wdia A \leq \cnomm_0, \bbox \cnomm_0 \leq \cnomm_2 \vd \wbox \cnomm_2 \geq \nomj_3$}
\DP
 \\
\end{tabular}
\end{center}
}

{\small
\begin{center}
\begin{tabular}{c}
\rotatebox[origin=c]{-90}{$\rightsquigarrow$} \rule[-2mm]{0mm}{6mm}\\
$\pi_2'$: Policy (2) where a renaming of term variables is needed in the second branch \\
exactly one cut formula is principal \\
\hline
\rule[0mm]{0mm}{32mm}
\AXC{$\pi_{2.1}$}
\RL{\fns Id$_{\,A \leq \cnomm_0}$}
\UIC{$A \leq \cnomm_0 \vd \cnomm_0 \geq A$}
\LL{\fns $\wbox_P$}
\UIC{$\nomj_1 \leq \wbox A, A \leq \cnomm_0 \vd \wbox \cnomm_0 \geq \nomj_1$}
\RL{\fns $\wbox_S$}
\UIC{$\nomj_1 \leq \wbox A \vd \textcolor{red}{\wbox A \geq \nomj_1}$}
%
\AXC{$\pi'_{2.2} = \pi_{2.2}[\nomj_1 \slash \nomj_3]$}
\RL{\fns Id$_{\,A\leq\cnomm_0}$}
\UIC{$A \leq \cnomm_0 \vd \cnomm_0 \geq A$}
\LL{\fns $\wbox_L$}
\UIC{$\textcolor{red}{\nomj_1 \leq \wbox A}, A \leq \cnomm_0 \vd \wbox \cnomm_0 \geq \nomj_1$}
\RL{\fns $\bdia \dashv \wbox$}
\UIC{$\textcolor{red}{\nomj_1 \leq \wbox A}, A \leq \cnomm_0 \vd \cnomm_0 \geq \bdia \nomj_1$}
\RL{\fns S}
\UIC{$\nomj_3 \leq \bdia \nomj_1, \textcolor{red}{\nomj_1 \leq \wbox A} \vd A \geq \nomj_3$}
\RL{\fns $\wdia_R$}
\UIC{$\nomj_3 \leq \bdia \nomj_1, \textcolor{red}{\nomj_1 \leq \wbox A}, \wdia A \leq \cnomm_0 \vd \cnomm_0 \geq \wdia \nomj_3$}
\LL{\fns $\wdia \dashv \bbox$}
\UIC{$\nomj_3 \leq \bdia \nomj_1, \textcolor{red}{\nomj_1 \leq \wbox A}, \wdia A \leq \cnomm_0 \vd \bbox \cnomm_0 \geq \nomj_3$}
\RL{\fns S}
\UIC{$\textcolor{red}{\nomj_1 \leq \wbox A}, \wdia A \leq \cnomm_0, \bbox \cnomm_0 \leq \cnomm_2 \vd \cnomm_2 \geq \bdia \nomj_1$}
\LL{\fns $\bdia \dashv \wbox^{-1}$}
\UIC{$\textcolor{red}{\nomj_1 \leq \wbox A}, \wdia A \leq \cnomm_0, \bbox \cnomm_0 \leq \cnomm_2 \vd \wbox \cnomm_2 \geq \nomj_1$}
%
\RL{\fns Cut$_{\,\nomj_1 \leq \wbox A}$}
\BIC{$\nomj_1 \leq \wbox A, \wdia A \leq \cnomm_0, \bbox \cnomm_0 \leq \cnomm_2 \vd \wbox \cnomm_2 \geq \nomj_1$}
\RL{\fns S}
\UIC{$\wdia A \leq \cnomm_0, \bbox \cnomm_0 \leq \cnomm_2, \wbox \cnomm_2 \leq \cnomm_4 \vd \cnomm_4 \geq \wbox A$}
\LL{\fns $\wbox_P$}
\UIC{$\nomj_3 \leq \wbox \wbox A, \wdia A \leq \cnomm_0, \bbox \cnomm_0 \leq \cnomm_2, \wbox \cnomm_2 \leq \cnomm_4 \vd \wbox \cnomm_4 \geq \nomj_3$}
\RL{\fns $\bdia \dashv \wbox$}
\UIC{$\nomj_3 \leq \wbox \wbox A, \wdia A \leq \cnomm_0, \bbox \cnomm_0 \leq \cnomm_2, \wbox \cnomm_2 \leq \cnomm_4 \vd \cnomm_4 \geq \bdia \nomj_3$}
\RL{\fns S}
\UIC{$\nomj_1 \leq \bdia \nomj_3, \nomj_3 \leq \wbox \wbox A, \wdia A \leq \cnomm_0, \bbox \cnomm_0 \leq \cnomm_2 \vd \wbox \cnomm_2 \geq \nomj_1$}
\DP
 \\
\end{tabular}
\end{center}
}

Notice that $s \neq s'$, where $s$ and $s'$ are the end-sequents of $\pi_2$ and $\pi_2'$, respectively. However, it is the case that $s \equiv s'$, modulo a global renaming of the nominals occurring in $\pi_2'$, namely $\pi_2 = \pi_2'\,[\nomj_3 \slash \nomj_1, \, \nomj_1 \slash \nomj_3]$.

If we consider initial rules with empty contexts and non-invertible logical rules, Policy (1) and Policy (2) are both correct and always applicable (this is essentially due to Proposition \ref{thm:SingleConclusion}). In particular, in Section \ref{ALIsAProperLabelledCalculus} we implemented the preservation of principal formulas's approximants along derivations (see Lemma \ref{thm:PreservationOfPrincipalFormulasApproximants}), namely Policy (1).

On the other hand, if we consider initial rules with non-empty contexts and invertible logical rules, Policy (1) and Policy (2) are not anymore interchangeable. Indeed, we might have multiple occurrences of labelled formulas in $\textrm{ant}(s)$ or in $\textrm{con}(s)$, where $s$ is a $\mathbf{A.L}\Sigma$-derivable sequent (so, Proposition \ref{thm:SingleConclusion} is not anymore valid). 

If we apply Policy (2) in the presence of non-empty contexts and invertible logical rules, we might run into some difficulties. Below we derive the proof section ending in the first premise of cut in the original proof. Notice how the side condition on the conclusion and on the premise of switch rules are violated in the application S$^{\star\star}$.

{\small
\begin{center}
\AXC{$\pi'_{2.1}$}
\RL{\fns Id$_{\,A\leq\cnomm_0}$}
\UIC{$\nomj_1 \leq \wbox \wbox A, \nomj_1 \leq \wbox A, A \leq \cnomm_0 \vd \cnomm_0 \geq A, \wbox \cnomm_0 \geq \nomj_1, \wbox \cnomm_2 \geq \nomj_1$}
\LL{\fns $\wbox_P$}
\UIC{$\nomj_1 \leq \wbox \wbox A, \nomj_1 \leq \wbox A, A \leq \cnomm_0 \vd \wbox \cnomm_0 \geq \nomj_1, \wbox \cnomm_2 \geq \nomj_1$}
\RL{\fns $\wbox_S$}
\UIC{$\nomj_1 \leq \wbox \wbox A, \nomj_1 \leq \wbox A \vd \textcolor{red}{\wbox A \geq \nomj_1}, \wbox \cnomm_2 \geq \nomj_1$}
\RL{\fns S$^{\star\star}$}
\UIC{$\nomj_1 \leq \wbox \wbox A, \textcolor{red}{\wbox A \leq \cnomm_2} \vd \cnomm_2 \geq \wbox A, \wbox \cnomm_2 \geq \nomj_1$}
\LL{\fns $\wbox_P$}
\UIC{$\nomj_1 \leq \wbox \wbox A, \textcolor{red}{\wbox A \leq \cnomm_2} \vd \wbox \cnomm_2 \geq \nomj_1$}
\RL{\fns $\bdia \dashv \wbox$}
\UIC{$\nomj_1 \leq \wbox \wbox A, \textcolor{red}{\wbox A \leq \cnomm_2} \vd \cnomm_2 \geq \bdia \nomj_1$}
\RL{\fns S}
\UIC{$\nomj_3 \leq \bdia \nomj_1, \nomj_1 \leq \wbox \wbox A \vd \textcolor{red}{\wbox A \geq \nomj_3} $}
\UIC{$\vdots$}
\DP
\end{center}
}

If we apply Policy (1) (namely, $\wbox_P, \wdia_S$ pick fresh nominals or conominals in the branch) in the presence of non-empty contexts and invertible logical rules, we might run into some difficulties as well. Nonetheless, we can solve the issue by relaxing the side conditions on switch rules, namely, dropping the side condition on the conclusion (which is not required for proving the soundness of switch rules) and retaining only the side condition on the premise.\footnote{To be proved rigorously.} Below we derive the proof section ending in the first premise of cut in the original proof. Notice how only the side condition on the conclusion of switch rules is violated in the application S$^\star$.

{\small
\begin{center}
\AXC{$\pi_{1.1}$}
\RL{\fns Id$_{\,A\leq\cnomm_0}$}
\UIC{$\nomj_3 \leq \wbox \wbox A, \nomj_1 \leq \wbox A, A \leq \cnomm_0 \vd \cnomm_0 \geq A, \wbox \cnomm_0 \geq \nomj_1, \wbox \cnomm_0 \geq \nomj_3$}
\LL{\fns $\wbox_P$}
\UIC{$\nomj_3 \leq \wbox \wbox A, \nomj_1 \leq \wbox A, A \leq \cnomm_0 \vd \wbox \cnomm_0 \geq \nomj_1, \wbox \cnomm_0 \geq \nomj_3$}
\RL{\fns $\wbox_S$}
\UIC{$\nomj_3 \leq \wbox \wbox A, \nomj_1 \leq \wbox A \vd \textcolor{red}{\wbox A \geq \nomj_1}, \wbox \cnomm_0 \geq \nomj_3$}
\RL{\fns S$^\star$}
\UIC{$\nomj_3 \leq \wbox \wbox A, \textcolor{red}{\wbox A \leq \cnomm_0} \vd \cnomm_0 \geq \wbox A, \wbox \cnomm_0 \geq \nomj_3$}
\LL{\fns $\wbox_P$}
\UIC{$\nomj_3 \leq \wbox \wbox A, \textcolor{red}{\wbox A \leq \cnomm_0} \vd \wbox \cnomm_0 \geq \nomj_3$}
\RL{\fns $\bdia \dashv \wbox$}
\UIC{$\nomj_3 \leq \wbox \wbox A, \textcolor{red}{\wbox A \leq \cnomm_0} \vd \cnomm_0 \geq \bdia \nomj_3$}
\RL{\fns S}
\UIC{$\nomj_1 \leq \bdia \nomj_3, \nomj_3 \leq \wbox \wbox A \vd \textcolor{red}{\wbox A \geq \nomj_1} $}
\UIC{$\vdots$}
\DP
\end{center}
}

Finally, we observe that in this case we might have derivable sequent $s = \Gamma \vdash \Delta$ where two formulas in $\Gamma$ (resp.~$\Delta$) are approximated by the same nominal or conominal (see for instance the initial sequent in the previous derivation, where $\{\nomj_3 \leq \wbox \wbox A, \nomj_1 \leq \wbox A\} \in \Gamma$). In similar cases we cannot immediately conjoin $\nomj_3 \leq \wbox \wbox A$ and $\nomj_1 \leq \wbox A$ by $\aand_P$ (no matter if we choose invertible or non-invertible logical rules). Nonetheless, the interpretation of sequents stay the same, namely $(\Gamma \vdash \Delta)^{\mathcal{A}} = \bigwedge^{\mathcal{A}} \Gamma^{\mathcal{A}} \Rarr \bigvee^{\mathcal{A}} \Delta^{\mathcal{A}}$. Notice that the following unary rules are sound as well:
{\small
\begin{center}
\begin{tabular}{rl}
\AXC{$\Gamma, \nomj_k \leq A, \nomj_\ell \leq B, \Gamma' \vd \Delta$}
\LL{$\aand_P$}
\UIC{$\Gamma, \nomj_k \aand \nomj_\ell \leq A \aand B, \Gamma' \vd \Delta$}
\DP
 \ & \  
\AXC{$\Gamma, A \leq \cnomm_k, B \leq \cnomm_\ell, \Gamma' \vd \Delta$}
\RL{$\aor_S$}
\UIC{$\Gamma, A \aor B \leq \cnomm_k \aor \cnomm_\ell, \Gamma' \vd \Delta$}
\DP
 \\
\mc{2}{c}{\rule[0mm]{0mm}{6mm} \fns ${}^\ast$Side condition: labelled formula in the conclusion are in display.} \\
\end{tabular}
\end{center}
 }

However, $\nomj_k \aand \nomj_\ell$ (resp.~$\cnomm_k \aor \cnomm_\ell$) is not necessarily a nominal (resp.~conominal).


\subsection{Canonical sequents and display property}

First, we fix the notation.

\begin{remark}[Notation]
\label{rem:SequencesOfStructures}
In what follows, we use 
\begin{itemize}
\item $\textrm{prem}(R)$ to denote the set of premises of $R$, which is either empty, a singleton, or contains two elements;
\item $\textrm{con}(R)$ to denote the set of conclusions of $R$, which is a singleton;
\item $s' = \sigma \cup s$ denotes the sequent $s$ expanded with the structure $\sigma$ (where $\sigma$ might occur in any position in $s'$);
\item $s' = \sigma, s$ (resp.~$s, \sigma$) denotes the sequent $s$ prefixed (resp.~suffixed) with the structure $\sigma$;
\item $\textrm{ant}(s)$ (resp.~$\textrm{con}(s)$) denotes the antecedent (resp.~consequent) of $s$;
\item $\textrm{sub}(x)$ denotes the set of subterms or subformulas of $x$;
\item $x, y , x', y'$ are either well-formed formulas or well-formed terms;
\item $|s|_n$ to denote a sequent $s$ contains exactly $n$ structures;
\end{itemize}
If $s = \Gamma \vdash \Delta$ is a derivable sequent and $\sigma = x \leq y \in \Delta$, where $x,y$ are well-formed terms or formulas, we  equivalently rewrite $\sigma$ in the following form $\sigma = y \geq x$.
\end{remark}

We now provide the definition of {\em canonical sequents}. Notice that this definition works whenever we consider initial rules with empty contexts and non-invertible logical rules. For dealing with initial rules with non-empty contexts and invertible logical rules, we will introduce {\em generalized canonical sequents}.

\begin{definition}[Canonical sequents]
\label{def:CanonicalSequents}
Two well-formed structures $\sigma = x R y$ and $ \sigma' = x' R y'$ occurring in a $\mathbf{A.L}\Sigma $-sequent $s$ are
\begin{itemize}
%\item there exists $s'$ s.t.~$s$ and $s'$ are equivalent modulo rearranging the order of structures in the antecedent;
\item {\em adjacent} iff $R = \,\leq$ if occurring in $\textrm{ant}(s)$, $R = \,\geq$ if occurring in $\textrm{con}(s)$, and $s$ has one of the following forms:
\subitem $s_a = \Gamma, \sigma, \sigma' \Gamma' \vdash \Delta$
\subitem $s_b = \Gamma, \sigma \vdash \sigma'$
\subitem $s_c = \sigma, \Gamma \vdash \sigma'$ 
\item {\em in connection} iff they are adjacent, and $\sigma, \sigma'$ are s.t.~at least one of the following is the case
\subitem $s \in \{s_a, s_b, s_c\}$ and $\abot \in \sigma'' \in \textrm{pre}(s)$ (resp.~$\aatop \in \sigma'' \in \textrm{suc}(s)$) where $\sigma'' \in \{\sigma,\sigma'\}$
\subitem $s \in \{s_a, s_b\}$ and $\textrm{sub}(y) \cap \textrm{sub}(x') \neq \emptyset$
\subitem $s = s_c$ and $\textrm{sub}(y') \cap \textrm{sub}(x) \neq \emptyset$
\item {\em in composition} iff they are in connection whenever adjacent.
\end{itemize}

A sequent $|s|_n$ is in {\em canonical form} (or simply {\em canonical}) iff $s$ is a {\em cycle} of the form

\begin{center}
$x_{1.1} \leq x_{1.2}, \ x_{2.1} \leq x_{2.2}, \ \ldots, \ x_{n-2.1} \leq x_{n-2.2}, \ x_{n-1.1} \leq x_{n-1.2} \ \vdash \ x_{n.1} \geq x_{n.2}$
\end{center}

\noindent and the adjacent structures occurring in $s$ are in composition.

A derivation $\pi$ is {\em in canonical form} iff for every sequent $s \in \pi$, $s$ is canonical.
\end{definition}



\begin{comment}
The following proposition would be valid only if we implement Policy (2).
\begin{lemma}
For every $\mathbf{A.L}\Sigma$-derivable sequent $s$, 
\begin{itemize}
\item if two labelled formulas $\{a_1, a_2\} \in \textrm{ant}(s)$ (resp.~$\{a_1, a_2\} \in \textrm{con}(s)$), then they share the very same term (which is an atomic term, namely the term approximant of the formulas occurring either in $a_1$ or in $a_2$);
\item if two pure structures $\{t_1, t_2\} \in \textrm{ant}(s)$ (resp.~$\{t_1, t_2\} \in \textrm{con}(s)$), $x_k, x_\ell$ are atomic terms, $x_k \in t_1$ and $x_\ell \in t_2$, then $k = \ell$.
\end{itemize}
\end{lemma}
\end{comment}

\begin{definition}
\label{def:SwitchPosition}
Two structures $\sigma, \sigma'$ are {\em twins} (or in {\em switch position}) in a canonical sequent $|s|_n$  iff $s$ has one of the following shape
\begin{itemize} 
\item $s_1 = \sigma, \Gamma \vdash \sigma'$
\item $s_{n-1} = \Gamma, \sigma \vdash \sigma'$
\end{itemize}
Morever, $\sigma, \sigma'$ are called 
\begin{itemize}
\item {\em $\nomj$-twins} if $\sigma = \nomj \leq x$ and $\sigma' = y \geq \nomj$ 
\item {\em $\cnomm$-twins} if $\sigma = x \leq \cnomm$ and $\sigma' = \cnomm \geq y$. 
\end{itemize}
\end{definition}

\begin{remark}[Notation]
\label{rem:Components}
Given a structure $\sigma = x R y$, $x, y$ are called {\em components}. If $\sigma, \sigma'$ are in connection, we write $\sigma_z, \prescript{}{z}\sigma'$ to signify that the that $z$ is the maximal non-empty intersection between the subcomponents of last component of $\sigma$ and the first component of $\sigma'$ or $z' \in \{\abot, \aatop\}$ for some $z' \in \textrm{sub}(z)$. We generalize the convention to meta-structures and canonical sequents as follows: $\prescript{}{x}\Gamma_y, \prescript{}{y}\Gamma'_z \vd \prescript{}{z}\Delta_w, \prescript{}{w}\Delta'_x$, where $\prescript{}{x}\Sigma_y = x R z, \Sigma', w R y$ for some structures $\sigma = x R z, \sigma' = w R y$ and form some list of structures $\Sigma'$ (where, if $\Sigma' = \emptyset$ then $z = w$). 
\end{remark}

We now prove the following result:\footnote{Notice that, modulo the equivalent rewriting in Remark \ref{rem:SequencesOfStructures}, every $\mathbf{A.L}\Sigma$-derivation occurring in the present paper is already in canonical form according to Definition \ref{def:CanonicalSequents}.}

\begin{lemma}[Canonical form]
\label{thm:CanonicalForm}
For every sequent $s$ occurring in an $\mathbf{A.L}\Sigma$-derivation $\pi$, there exists an equivalent (modulo a reordering of structures) sequent $s'$ that is in canonical form (see Definition \ref{def:CanonicalSequents}), and the derivation $\pi'= \pi[s' \slash s]$.
\end{lemma}

\begin{proof}
The proof is by induction on the height of derivations. It is enough to show that if every premise of a rule $R \in \mathbf{A.L}\Sigma$ is in canonical form, then the conclusion of $R$ is in canonical form. 

\paragraph{$R$ is an initial rule.} Initial rules $R$ do not have premises, so it is enough to check that the conclusion of $R$ is in canonical form, but this is immediate to see by inspecting all initial rules.

{\small
\vspace{-0.25cm}
\begin{center}
\begin{tabular}{rl}
\AXC{$ \ $}
\LL{Id$_{\,\nomj \leq p}$}
\UIC{$\nomj \leq p \vd p \geq \nomj$}
\DP
 \ \,
\AXC{$\ $}
\RL{Id$_{\,p \leq \cnomm}$}
\UIC{$p \leq \cnomm \vd \cnomm \geq p$}
\DP 

\  & \ 
 
\AXC{ \ }
\LL{\fns Id$_{\abot}$}
\UIC{$\bot \leq \cnomm \vd \cnomm \geq \abot$}
\DP
 \ \,
\AXC{ \ }
\RL{\fns Id$_{\aatop}$}
\UIC{$\nomj \leq \top \vd \aatop \geq \nomj$}
\DP
 \\

 & \\

\AXC{ \ }
\LL{\fns $\abot_{W}$}
\UIC{$p \leq \cnomm \vd \cnomm \geq \abot$}
\DP
 \ & \
\AXC{ \ }
\RL{\fns $\aatop_{W}$}
\UIC{$\nomj \leq p \vd \aatop \geq \nomj$}
\DP
 \\
\end{tabular}
\end{center}
}

In what follows we present the rules of $\mathbf{A.L}\Sigma$ in a specific format, namely we appropriately rearrange the sequence of structures occurring in $\textrm{ant}(s)$ (resp.~in $\textrm{ant}(s)$), where $s$ is a premise or the consequence of a rule. Notice that rules in this format are equivalent to the original ones, given that commas occurring in sequents are commutative and associative. By inspecting the shape of the rules in the new format, it is immediate to see that if the premises are canonical, then also the conclusion is canonical. To emphasize why this is the case, we use the notational convention of Remark \ref{rem:Components}.

\paragraph{$R$ is a logical rule for propositional connectives.} 

Below we equivalently reformulate the logical rules introducing propositional connectives. %We use the notation $\sigma \cup \Gamma$ to signify that the parametric labelled formulas in the conclusion of these rules occur in the very same position as the parametric labelled formulas in the premise, whichever the position is.
Notice that:
\begin{itemize}
\item if $s$ is the conclusion of $\aand_P$ (resp.~$\aor_S$), then the principal structure occurs in first (resp.~last) position in $\textrm{ant}(s)$;
\item if $s$ is the conclusion of $\aand_S$ (resp.~$\aor_P$), then the principal structure occurs in last (resp.~first) position in $\textrm{con}(s)$.
\end{itemize}

{\small
\begin{center}
\begin{tabular}{rl}
\AXC{$\nomj \leq  A, \, \prescript{}{A}\Gamma_x \vd\! \prescript{}{x\,}\Delta_{\,\nomj}$}
\LL{$\aand_{P1}$}
\UIC{$\nomj \leq A \aand B, \, \prescript{}{A}\Gamma_x \vd\! \prescript{}{x\,}\Delta_{\,\nomj}$}
\DP
 \ & \
 \\

& \\

\AXC{$\nomj \leq  B, \, \prescript{}{B}\Gamma_x \vd\! \prescript{}{x\,}\Delta_{\,\nomj}$}
\LL{$\aand_{P2}$}
\UIC{$\nomj \leq A \aand B, \, \prescript{}{B}\Gamma_x \vd\! \prescript{}{x\,}\Delta_{\,\nomj}$}
\DP
 \ & \ 
\AXC{$\prescript{}{\nomj}\Gamma_x \vd\! \prescript{}{x\,}\Delta_y, \, \prescript{}{y\,}A 
\geq \nomj$}
\AXC{$\prescript{}{\nomj}\Gamma_x \vd\! \prescript{}{x\,}\Delta_y, \, \prescript{}{y\,}B \geq \nomj$}
\RL{$\aand_S$}
\BIC{$\prescript{}{\nomj}\Gamma_x \vd\! \prescript{}{x\,}\Delta_y, \, A \aand B \geq \nomj$}
\DP
 \\

 & \\
 
\AXC{$\prescript{}{x\,}\Gamma_{\cnomm} \vd \cnomm \geq A_y, \, \prescript{}{y\,}\Delta_{x}$}
\AXC{$\prescript{}{x}\Gamma_{\cnomm} \vd \cnomm \geq B_y, \, \prescript{}{y\,}\Delta_{x}$}
\LL{$\aor_{P}$}
\BIC{$\prescript{}{x\,}\Gamma_{\cnomm} \vd \cnomm \geq A \aor B_y, \, \prescript{}{y\,}\Delta_{x}$}
\DP
 \ & \  
\AXC{$\prescript{}{x\,}\Gamma_{A}, \, A \leq \cnomm \vd\! \prescript{}{\cnomm\,}\Delta_x$}
\RL{$\aor_{S1}$}
\UIC{$\prescript{}{x\,}\Gamma_{A}, \,  A \aor B \leq \cnomm \vd\! \prescript{}{\cnomm\,}\Delta_x$}
\DP
\\

& \\

 \ & \ 
\AXC{$\prescript{}{x\,}\Gamma_{B}, \, B \leq \cnomm \vd\! \prescript{}{\cnomm\,}\Delta_x$}
\RL{$\aor_{S2}$}
\UIC{$\prescript{}{x\,}\Gamma_{B}, \,  A \aor B \leq \cnomm \vd\! \prescript{}{\cnomm\,}\Delta_x$}
\DP
 \\
\mc{2}{c}{\rule[0mm]{0mm}{6mm} \fns ${}^\ast$Side condition: labelled formula in the conclusion of any logical rule are in display.} \\
\end{tabular}
\end{center}
 }

\begin{comment}
We consider $R = \aand_S$. If $s_1, s_2 \in \textrm{prem}(R)$, and $s_3 \in \textrm{con}(R)$, then $|s_1|_n = |s_2|_n = |s_3|_n$. For every $i \in \{1,2\}$, we observe that:
(a) $s_3 = s_i [x_3 R y_3 \slash x_i R y_i]$, where $x_3 R y_3 \in \textrm{con}(s_3)$ and $x_i R y_i \in \textrm{con}(s_i)$ are the nonparametric structures of $R$; (b) $\textrm{sub}(y_i) \cap \textrm{sub}(y_3) \neq \emptyset$, given that $y_1 = y_2 = y_3 = \nomj$ for some nominal $\nomj$; (c) $\textrm{sub}(x_i) \cap \textrm{sub}(x_3) \neq \emptyset$, given that $x_1 = A_1$ and $x_2 = A_2$ (for some formulas $A_1, A_2$) are the immediate subformulas of the (principal) formula $x_3 = A_1 \aand A_2$. (a) ensures that, modulo substituting $x_3 R y_3$ for $x_i R y_i$, $s_3$ is the very same sequence of structures as $s_i$, so (b) and (c) guarantee that adjacent structures remain in connection. Therefore, $s_3$ is canonical whenever $s_1$ and $s_2$ are canonical. 

We consider $R = \aand_P$. If $s_1 \in \textrm{prem}(R)$, and $s_2 \in \textrm{con}(R)$, then $|s_1|_n = |s_2|_n$. We observe that:
(a) $s_2 = s_1 [x_2 R y_2 \slash x_1 R y_1]$, where $x_2 R y_2 \in \textrm{ant}(s_2)$ and $x_1 R y_1 \in \textrm{ant}(s_1)$ are the nonparametric structures of $R$; (b) $\textrm{sub}(x_1) \cap \textrm{sub}(x_2) \neq \emptyset$, given that $x_1 = x_2 = \nomj$ for some nominal $\nomj$; (c) $\textrm{sub}(y_1) \cap \textrm{sub}(y_2) \neq \emptyset$, given that $y_1 = A_i$ (for some formula $A_i \in \{A_1, A_2\}$) is an immediate subformula of the (principal) formula $y_2 = A_1 \aand A_2$. (a) ensures that, modulo substituting $x_2 R y_2$ for $x_1 R y_1$, $s_2$ is the very same sequence of structures as $s_1$, so (b) and (c) guarantee that adjacent structures remain in connection. Therefore, $s_2$ is canonical whenever $s_1$ is canonical. 

If $R = \aor_P$ or $R = \aor_S$, the reasoning is similar and we omit it.
\end{comment}

\paragraph{$R$ is a logical rule for modalities.} 

Below we equivalently reformulate the logical rules introducing modalities. Notice that:
\begin{itemize}
\item if $s$ is the conclusion of $\wbox_P$ (resp.~$\wdia_S$), then the principal structure occurs in first (resp.~last) position in $\textrm{ant}(s)$, and the other nonparametric structure occurs in the last (resp.~first) position in $\textrm{con}(s)$;
\item if $s$ is the conclusion of $\wbox_S$ (resp.~$\wdia_P$), then the principal structure occurs in first (resp.~last) position in $\textrm{con}(s)$.
\end{itemize}

{\small
\begin{center}
\begin{tabular}{rl}
\AXC{$\prescript{}{A}\Gamma_x \vd\! \prescript{}{x\,}\Delta_\cnomm, \, \cnomm \geq A$}
\LL{$\wbox_P$}
\UIC{$\nomj \leq \wbox A, \prescript{}{A}\Gamma_x \vd\! \prescript{}{x\,}\Delta_\cnomm, \, \wbox \cnomm \geq \nomj$}
\DP 
 \ & \  
\AXC{$\prescript{}{x\,}\Gamma_A, \, A \leq \cnomm \vd \wbox \cnomm \geq \nomj, \prescript{}{\nomj\,}\Delta_x$}
\RL{$\wbox_S$}
\UIC{$\prescript{}{x\,}\Gamma_A \vd \wbox A \geq \nomj, \prescript{}{\nomj\,}\Delta_x$}
\DP
 \\

 & \\

\AXC{$\nomj \leq A, \, \prescript{}{A\,}\Gamma_x \vd\! \prescript{}{x\,}\Delta_{\cnomm}, \, \cnomm \geq \wdia \nomj$}
\LL{$\wdia_P$}
\UIC{$\prescript{}{A\,}\Gamma_x \vd\! \prescript{}{x\,}\Delta_{\cnomm}, \, \cnomm \geq \wdia A$}
\DP
 \ & \ 
\AXC{$\prescript{}{x\,}\Gamma_A \vd A \geq \nomj, \, \prescript{}{\nomj\,}\Delta_x$}
\RL{$\wdia_S$}
\UIC{$\prescript{}{x\,}\Gamma_A, \, \wdia A \leq \cnomm \vd \cnomm \geq \wdia \nomj, \prescript{}{\nomj\,}\Delta_x$}
\DP  
 \\
\end{tabular}
\begin{tabular}{rl}
\mc{2}{c}{\rule[0mm]{0mm}{6mm} \fns $^\ast$Side conditions: $\cnomm$ (resp.~$\nomj$) must not occur in the conclusion of $\wbox_S$ (resp.~$\wdia_P$).} \\
\mc{2}{c}{\fns Labelled formulas in the conclusion of any logical rule are in display.} \\
\end{tabular}
\end{center}
 }

\begin{comment}
We consider $R = \wbox_P$. If $s_1 \in \textrm{prem}(R)$, and $s_2 \in \textrm{con}(R)$, then $|s_1|_n$ and $|s_2|_{n+1}$. We observe that:
(a) $s_2 = x_2 R y_2, s_2'$ and $s_2' = s_1 [x_3 R y_3 \slash x_1 R y_1]$, $x_2 R y_2 \in \textrm{ant}(s_2)$, $x_3 R y_3 \in \textrm{con}(s_2)$ and $x_1 R y_1 \in \textrm{con}(s_1)$ are the nonparametric structures of $R$, and $x_2 R y_2$ contains the principal formula of $R$; (b) $\textrm{sub}(x_1) \cap \textrm{sub}(x_3) \neq \emptyset$, given that $x_1 = \cnomm$ for some conominal $\cnomm$ and $x_3 = \wbox x_1$; (c) $\textrm{sub}(y_1) \cap \textrm{sub}(y_2) \neq \emptyset$, given that $y_1 = A$ (for some formula $A$) is the immediate subformula of the (principal) formula $y_2 = \wbox A$. (a) ensures that, modulo substituting $x_3 R y_3$ for $x_1 R y_1$, $s_2'$ is the very same sequence of structures as $s_1$, so (b) and (c) guarantee that adjacent structures in $s_1$ remain in connection in $s_2$ (given that $s_2 = x_3 R y_3, s_2'$). Therefore, $s_2$ is canonical whenever $s_1$ is canonical.
\end{comment}


\paragraph{$R$ is an adjunction rule.}

{\small
\begin{center}
\begin{tabular}{rl}

\AXC{$\prescript{}{x\,}\Gamma_\cnomm \vd \cnomm \geq \wdia \nomj, \, \prescript{}{\nomj\,}\Delta_x$}
\LL{\fns $\wdia \dashv \bbox$}
\UIC{$\prescript{}{x\,}\Gamma_\cnomm \vd \bbox \cnomm \geq \nomj, \, \prescript{}{\nomj\,}\Delta_x$}
\DP 
 \ & \  
\AXC{$\prescript{}{x\,}\Gamma_\cnomm \vd \bbox \cnomm \geq \nomj, \, \prescript{}{\nomj\,}\Delta_x$}
\RL{\fns $\wdia \dashv \bbox^{-1}$}
\UIC{$\prescript{}{x\,}\Gamma_\cnomm \vd \cnomm \geq \wdia \nomj, \, \prescript{}{\nomj\,}\Delta_x$}
\DP
 \\

 & \\
 
\AXC{$\prescript{}{x\,}\Gamma_\cnomm \vd \wbox \cnomm\geq \nomj, \, \prescript{}{\nomj\,}\Delta_x$}
\LL{\fns $\bdia \dashv \wbox$}
\UIC{$\prescript{}{x\,}\Gamma_\cnomm \vd \cnomm\geq \bdia\nomj, \, \prescript{}{\nomj\,}\Delta_x$}
\DP 
 \ & \  
\AXC{$\prescript{}{x\,}\Gamma_\cnomm \vd \cnomm\geq \bdia\nomj, \, \prescript{}{\nomj\,}\Delta_x$}
\RL{\fns $\bdia \dashv \wbox^{-1}$}
\UIC{$\prescript{}{x\,}\Gamma_\cnomm \vd \wbox \cnomm\geq \nomj, \, \prescript{}{\nomj\,}\Delta_x$}
\DP
 \\
\end{tabular}
\end{center}
 }

\paragraph{$R$ is a structural rule for $\aatop$ and $\abot$.}

{\small
\begin{center}
\begin{tabular}{rl}
\AXC{$\prescript{}{\aatop\,}\Gamma_{\,\cnomm} \vd \cnomm \geq \aatop$}
\LL{\fns $\aatop_\wbox$}
\UIC{$\nomj \leq \aatop, \, \prescript{}{\aatop\,}\Gamma_{\,\cnomm} \vd \wbox \cnomm\geq \nomj$}
\DP
 \ & \ 
\AXC{$\prescript{}{x\,}\Gamma_{\abot} \vd \abot \geq \nomj, \, \prescript{}{\nomj\,}\Delta_x$}
\RL{\fns $\abot_\wdia$}
\UIC{$\prescript{}{x\,}\Gamma_{\abot}, \, \abot \leq \cnomm \vd \cnomm \geq \wdia \nomj, \, \prescript{}{\nomj\,}\Delta_x$}
\DP
 \\
\end{tabular}
\end{center}
 }

\paragraph{$R$ is a cut rule.}

{\small
\begin{center}
\begin{tabular}{rl}
\AXC{$\prescript{}{x\,}\Gamma_A \vd A \geq \nomj, \,  \prescript{}{\nomj\,}\Delta_x$}
\AXC{$\nomj \leq A, \, \prescript{}{A\,}\Gamma'_y \vd\! \prescript{}{y\,}\Delta'_{\,\nomj}$}
\LL{Cut$_{\,\nomj\leq A}$}
\BIC{$\prescript{}{x\,}\Gamma_A, \, \prescript{}{A\,}\Gamma'_y \vd\! \prescript{}{y\,}\Delta'_{\,\nomj}, \, \prescript{}{\nomj\,}\Delta_x$}
\DP
 \ & \  
\AXC{$\prescript{}{A\,}\Gamma_x \vd\! \prescript{}{x\,}\Delta_{\, \cnomm}, \, \cnomm \geq A$}
\AXC{$\prescript{}{y\,}\Gamma'_A, \, A \leq \cnomm \vd\! \prescript{}{\cnomm\,}\Delta'_y$}
\RL{Cut$_{\,A\leq \cnomm}$}
\BIC{$\prescript{}{y\,}\Gamma'_A, \, \prescript{}{A\,}\Gamma_x \vd\! \prescript{}{x\,}\Delta_{\, \cnomm}, \, \prescript{}{\cnomm\,}\Delta'_y$}
\DP 
 \\
\mc{2}{c}{\rule[0mm]{0mm}{6mm} \fns ${}^\ast$Side condition: $\nomj \leq A$ and $A \leq \cnomm$ are in display.} \\ 
\mc{2}{c}{\fns  
} \\ 
\end{tabular}
\end{center}
 }

\paragraph{$R$ is a switch rule.}\marginnote{G: Here I need to relax the side condition on the conclusions of switch rule admitting multiple copies of labelled formulas approximated by the same nominal/conominal (but not pure structures approximated by the same nominal/conominal).}

{\small
\begin{center}
\begin{tabular}{rl}
%\rule[-1.85mm]{0mm}{8mm}
\AXC{$\nomj \leq A, \, \prescript{}{A\,}\Gamma_{\cnomm} \vd \cnomm \geq \nomj$}
\LL{\fns S$\cnomm$}
\UIC{$\prescript{}{A\,}\Gamma_{\, \cnomm} \vd \cnomm \geq A$}
\DP 
 \ & \ 
\AXC{$\prescript{}{\nomj\,}\Gamma_A, \, A \leq \cnomm \vd \cnomm \geq \nomj$}
\RL{\fns S$\nomj$}
\UIC{$\prescript{}{\nomj\,}\Gamma_A \vd A \geq \nomj$}
\DP 
 \\

 & \\

\AXC{$\nomj \leq  A, \, \prescript{}{A\,}\Gamma_B \vd B \geq \nomj$}
\LL{S$\cnomm\cnomm$}
\UIC{$\prescript{}{A\,}\Gamma_B, \, B \leq \cnomm \vd \cnomm \geq A$}
\DP
 \ & \ 
\AXC{$\prescript{}{B\,}\Gamma_A, \, A \leq \cnomm \vd \cnomm \geq B$}
\RL{S$\nomj\nomj$}
\UIC{$\nomj \leq  B, \, \prescript{}{B\,}\Gamma_A \vd A \geq \nomj$}
\DP
 \\

 & \\

\AXC{$\nomj \leq \NCT, \, \prescript{}{\NCT\,}\Gamma_A \vd A \geq \nomj$}
\LL{S$\cnomm\NCT$}
\UIC{$\prescript{}{\NCT\,}\Gamma_A, \, A \leq \cnomm \vd \cnomm \geq \NCT$}
\DP

 \ & \  

\AXC{$\prescript{}{A\,}\Gamma_{\NCT}, \, \NCT \leq \cnomm \vd  \cnomm \geq A$}
\RL{S$\nomj\NCT$}
\UIC{$\nomj \leq A, \, \prescript{}{A\,}\Gamma_{\NCT} \vd \NCT \geq \nomj$}
\DP

 \\

 & \\
\AXC{$\nomj \leq A, \, \prescript{}{A\,}\Gamma_{\NCT} \vd \NCT \geq \nomj$}
\LL{S$\NCT\cnomm$}
\UIC{$\prescript{}{A\,}\Gamma_{\NCT}, \, \NCT \leq \cnomm \vd \cnomm \geq A$}
\DP

 \ & \  

\AXC{$\prescript{}{\NCT\,}\Gamma_A, \, A \leq \cnomm \vd \cnomm \geq \NCT$}
\RL{S$\NCT\nomj$}
\UIC{$\nomj \leq \NCT, \, \prescript{}{\NCT\,}\Gamma_A \vd A \geq \nomj$}
\DP
 
 \\
 &\\
  \AXC{$\nomj \leq \NCT', \, \prescript{}{\NCT'\,}\Gamma_{\NCT} \vd \NCT \geq \nomj$}
\LL{S$\NCT\NCT'\cnomm$}
\UIC{$\prescript{}{\NCT'\,}\Gamma_{\NCT}, \, \NCT \leq \cnomm \vd \cnomm \geq \NCT'$}
\DP

 \ & \  

\AXC{$\prescript{}{\NCT\,}\Gamma_{\NCT'}, \, \NCT' \leq \cnomm \vd \cnomm \geq \NCT$}
\RL{S$\nomj\NCT\NCT'$}
\UIC{$\nomj \leq \NCT, \prescript{}{\NCT\,}\Gamma_{\NCT'} \vd \NCT' \geq \nomj$}
\DP
 \\
\mc{2}{c}{\rule[0mm]{0mm}{6mm} ${ }^\ast$Side condition: \fns{For all the switch rules except S$\cnomm$ and S$\nomj$,}} \\
\mc{2}{c}{\fns {$\nomj$ and $\cnomm$ do not appear in $\Gamma$ or $\Delta$. $\nomj$ (resp.~$\cnomm$) in S$\cnomm$ (resp.~S$\nomj$)}}\\
\mc{2}{c}{\fns {must not appear in the conclusion of the rule.}}
%  \mc{2}{c}{\rule[0mm]{0mm}{6mm} ${ }^\ast$Side condition: \fns{For all the rules except S$\cnomm$ and S$\nomj$ $\nomj$ and $\cnomm$ do not appear in $\Gamma$ or $\Delta$. }} \\
% \mc{2}{c}{\fns {$\nomj$ (resp.~$\cnomm$) in rule S$\cnomm$ (resp.~S$\nomj$) must not appear in conclusion of the rule. } }
% \mc{2}{c}{\fns $\cnomm$ in S$\NCT\NCT'\cnomm$ (resp.~$\nomj$ in S$\nomj\NCT\NCT'$) must not occur in $\Gamma, \Delta$.}
\end{tabular}
\end{center}
 }

\begin{remark}[Nomenclature]
\label{rem:(Anti-)ClockwiseSwitchRules}
If $\textrm{S} \in \{\textrm{S} _{\cnomm\cnomm}, \textrm{S}_{\cnomm\NCT}, \textrm{S}_{\NCT\cnomm}, \textrm{S}_{\NCT\NCT'\cnomm}\}$, we call $S$ {\em clockwise switch rule}. If $\textrm{S} \in \{\textrm{S} _{\nomj\nomj}, \textrm{S}_{\nomj\NCT}, \textrm{S}_{\NCT\nomj}, \textrm{S}_{\NCT\NCT'\cnomm}\}$, we call $S$ {\em anti-clockwise switch rule}.
\end{remark}

\paragraph{$R$ is a structural rule.} 

{\small
\begin{center}
\begin{tabular}{c}
\AXC{$\prescript{}{\nomj\,}\Gamma_{\cnomm} \vd \cnomm \geq \wdia \nomj$}
\LL{\fns $4$}
\UIC{$\nomh \leq \wdia \nomj, \, \prescript{}{\nomj\,}\Gamma_{\cnomm} \vd \cnomm \geq \wdia \nomh $}
\DP 
 \qquad 
\AXC{$\prescript{}{x\,}\Gamma_{\,\cnomm} \vd \wbox \cnomm \geq \nomj, \, \prescript{}{\nomj\,}\Delta_x$}
\RL{\fns $T$}
\UIC{$\prescript{}{x\,}\Gamma_{\,\cnomm} \vd \cnomm \geq \nomj, \, \prescript{}{\nomj\,}\Delta_x$}
\DP
 \qquad
\AXC{$\prescript{}{x\,}\Gamma_{\,\cnomm} \vd \cnomm \geq \wdia \nomj, \, \prescript{}{\nomj\,}\Delta_x$}
\RL{\fns $B$}
\UIC{$\prescript{}{x\,}\Gamma_{\,\cnomm} \vd \wbox \cnomm\geq\nomj, \, \prescript{}{\nomj\,}\Delta_x$}
\DP
 \\
   \\
\AXC{$\nomk \leq \bdia \nomj, \, \prescript{}{\nomj\,}\Gamma_{\,\cnomm} \vd \cnomm \geq \wdia \nomk$}
\RL{\fns D}
\UIC{$\prescript{}{\nomj\,}\Gamma_{\,\cnomm} \vd \cnomm \geq \nomj$}
\DP
 \qquad
\AXC{$\nomk \leq \bdia \nomj, \, \prescript{}{\nomj\,}\Gamma_{\,\cnomm} \vd \cnomm \geq \wdia \nomk$}
\RL{\fns $C$}
\UIC{$\nomh \leq \wdia \nomj, \, \prescript{}{\nomj\,}\Gamma_{\,\cnomm} \vd \cnomm \geq \bdia \nomh$}
\DP
 \\
\end{tabular}
\end{center}
 }
 
\end{proof}


\begin{lemma}[Cyclic permutations]
\label{thm:Permutation}
If $s = \Gamma \vd \Delta$ is a derivable sequent in canonical form and $\sigma \in \Gamma$ is a structure, then there exist a derivable sequent where $\sigma$ is in switch position (see Definition \ref{def:SwitchPosition}). That is, if $s \in \textrm{ant}(s)$, then there exist two sequents $s_1, s_{n-1}$ and two derivations $\pi_1, \pi_{n-1}$ s.t.
\begin{itemize}
\item $s_1 = \sigma_1, \Gamma' \vd \Delta'$, and $s_{n-1} = \Gamma', \sigma_{n-1} \vd \Delta'$;
\item $\pi_1$ and $\pi_{n-1}$ are constructed via $n$ applications of switch rules with $n \geq 0$;
\item $\pi$ (resp.~$\pi_{n-1}$) is a derivation of $s_1 $ (resp.~$s_{n-1}$) from $s$, and $\sigma, \sigma_1$ are congruent in $\pi_1$ (resp.~$\pi_{n-1}$), and $\sigma = \sigma_1 = \sigma_{n-1}$.
\end{itemize}
\end{lemma}

\begin{proof}
If $\sigma$ occurs in $\Gamma$ in the first (resp.~last) position, then $\pi_1 = s$ (resp.~$\pi_{n-1} = s)$. Otherwise, (a) $s = \sigma_1, \Gamma' \vdash \sigma_n, \Delta'$ or (b) $s = \Gamma', \sigma_{n-1}  \vdash \sigma_n, \Delta'$, where $\sigma \in \Gamma'$.

If $S$ is a {\em clockwise switch rule} (see Remark \ref{rem:(Anti-)ClockwiseSwitchRules}), then $S$ induces a 1-step clockwise cyclic permutation, namely the generic shape of $S$ is as follows:
\begin{center}
\AXC{$\sigma_1, \Gamma' \vdash \sigma_n, \Delta'$}
\LL{\fns S}
\UIC{$\Gamma', \sigma_n' \vdash \sigma_1', \Delta'$}
\DP
\end{center}
\noindent where $\textrm{prem}(\textrm{S})$ is of the form $(a)$ and $\sigma_1, \sigma_n$ (resp.~$\sigma_n', \sigma_1'$) are the nonparametric structures in $\textrm{prem}(\textrm{S})$ (resp.~$\textrm{con}(\textrm{S})$). It is immediate to see that, for each clockwise switch rules $S$, a parametric structure occurring in the antecedent (i.e.~$\sigma \in \Gamma'$) is 1-step closer to the first position when occurring in the conclusion (i.e.~$\sigma \in \textrm{con}(S)$) rather than when occurring in the premise (i.e.~$\sigma \in \textrm{pre}(S)$). Therefore, $\pi_1$ can be effectively constructed via a finite number of applications of clockwise switch rules.

If $S$ is a {\em anti-clockwise switch rule} (see Remark \ref{rem:(Anti-)ClockwiseSwitchRules}), then $S$ induces a 1-step anti-clockwise cyclic permutation, namely the generic shape of $S$ is as follows:
\begin{center}
\AXC{$\Gamma', \sigma_{n-1} \vdash \sigma_n, \Delta'$}
\RL{\fns S}
\UIC{$\sigma_n', \Gamma' \vdash \sigma_{n-1}', \Delta'$}
\DP
\end{center}
\noindent where $\textrm{prem}(\textrm{S})$ is of the form $(b)$ and $\sigma_{n-1}, \sigma_n$ (resp.~$\sigma_n', \sigma_{n-1}'$) are the nonparametric structures in $\textrm{prem}(\textrm{S})$ (resp.~$\textrm{con}(\textrm{S})$). It is immediate to see that, for each anti-clockwise switch rules $S$, a parametric structure in the antecedent (i.e.~$\sigma \in \Gamma'$) is 1-step closer to the last position when occurring in the conclusion (i.e.~$\sigma \in \textrm{con}(S)$) rather than when occurring in the premise (i.e.~$\sigma \in \textrm{pre}(S)$). Therefore, $\pi_{n-1}$ can be effectively constructed via a finite number of applications of anti-clockwise switch rules.
\end{proof}



\begin{lemma}[$\nomj$-twin (resp.~$\cnomm$-twin) structures are displayable]
\label{thm:Pre-inverse}
For every derivable canonical sequent $s$, if $s$ has one of the following forms
\begin{itemize}
\item ($\nomj$-twins) \ if $s = \nomj \leq x, \Gamma \vd y \geq \nomj$ and $\sigma \in \{\nomj \leq x, y \geq \nomj\}$
\item ($\cnomm$-twins) \ if $s = \Gamma, x \leq \cnomm \vd \cnomm \geq y$ and $\sigma \in \{x \leq \cnomm, \cnomm \geq y\}$
\end{itemize}
\noindent then, $\sigma$ is displayable with at most one application of switch $S$ (where $\sigma$ is a nonparametric structure of $S$) immediately followed by at most one application of adjunction.
\end{lemma}

\begin{proof}

\end{proof}

\begin{theorem}[Structures are displayable]
\label{thm:DisplayPropertyAL2}
If $s =\Gamma \vd \Delta $ is a derivable $\mathbf{A.L}\Sigma$-sequent, then every structure $\sigma$ occurring in $s$ is {\em displayable} (see Definition \ref{def:Display}).
\end{theorem}

\begin{proof}
By Lemma \ref{thm:CanonicalForm}, every derivable sequent can be presented in canonical form. By Lemma \ref{thm:Permutation}, if a structure $\sigma$ occurs in a canonical sequent $s$, then $\sigma$ is a twin structure in a canonical sequent $s'$ where $s'$ is derivable from $s$ via zero or more application of switch rules. 

For every derivable canonical sequent $s$ and every well-formed structure $\sigma$,
\begin{itemize}
\item if $\sigma \in \textrm{ant}(s)$, then $\sigma \in \{\nomj \leq z, \cnomm \leq z\}$
\item if $\sigma \in \textrm{con}(s)$, then $\sigma \in \{z \geq \nomj, z \geq \cnomm\}$.
\end{itemize}

\textcolor{red}{G: to be finished taking into account the relaxation of the side condition n the conclusion of switch rules.}

By Lemma \ref{thm:Pre-inverse}, every $\nomj$-twin (resp.~$\cnomm$-twin) structure is displayable. 
\label{thm:Permutation}

\end{proof}

\begin{comment}
{\small
\begin{flushright}
\AXC{$\pi'_{2.2}$}
\RL{\fns Id$_{\,A\leq\cnomm_0}$}
\UIC{$A \leq \cnomm_0 \vd \cnomm_0 \geq A$}
\LL{\fns $\wbox_L$}
\UIC{$\textcolor{red}{\nomj_3 \leq \wbox A}, A \leq \cnomm_0 \vd \wbox \cnomm_0 \geq \nomj_3$}
\RL{\fns $\bdia \dashv \wbox$}
\UIC{$\textcolor{red}{\nomj_3 \leq \wbox A}, A \leq \cnomm_0 \vd \cnomm_0 \geq \bdia \nomj_3$}
\RL{\fns S}
\UIC{$\nomj_5 \leq \bdia \nomj_3, \textcolor{red}{\nomj_3 \leq \wbox A} \vd A \geq \nomj_5$}
\RL{\fns $\wdia_R$}
\UIC{$\nomj_5 \leq \bdia \nomj_3, \textcolor{red}{\nomj_3 \leq \wbox A}, \wdia A \leq \cnomm_2 \vd \cnomm_2 \geq \wdia \nomj_5$}
\LL{\fns $\wdia \dashv \bbox$}
\UIC{$\nomj_5 \leq \bdia \nomj_3, \textcolor{red}{\nomj_3 \leq \wbox A}, \wdia A \leq \cnomm_2 \vd \bbox \cnomm_2 \geq \nomj_5$}
\RL{\fns S}
\UIC{$\textcolor{red}{\nomj_3 \leq \wbox A}, \wdia A \leq \cnomm_2, \bbox \cnomm_2 \leq \cnomm_4 \vd \cnomm_4 \geq \bdia \nomj_3$}
\LL{\fns $\bdia \dashv \wbox^{-1}$}
\UIC{$\textcolor{red}{\nomj_3 \leq \wbox A}, \wdia A \leq \cnomm_2, \bbox \cnomm_2 \leq \cnomm_4 \vd \wbox \cnomm_4 \geq \nomj_3$}
\UIC{[2]}
\DP
\end{flushright}
}

{\small
\begin{center}
\AXC{[1]\ \ \ \ \ \ \ \ \ \ }
\AXC{\ \ \ \ \ \ \ \ \ \ [2]}
\RL{\fns Cut$_{\,\nomj_3 \leq \wbox A}$}
\BIC{$\nomj_3 \leq \bdia \nomj_1, \nomj_1 \leq \wbox \wbox A, \wdia A \leq \cnomm_2, \bbox \cnomm_2 \leq \cnomm_4 \vd \wbox \cnomm_4 \geq \nomj_3$}
\DP
\end{center}
}
\end{comment}

%\input{Display&C6C7.tex}

==> SyntacticCompleteness-OLDVersion.tex <==
\subsection{Completeness}

\textcolor{red}{G: Notice that the display the labelled derivation are exactly the same modulo switch rules $S$.}


\paragraph{\textbf{Transitivity.}}

Let us consider the axiom $(4)\  \wdia \wdia A \vdash \wdia A$. Using ALBA we generate the first order correspondent:

\begin{center}
$\forall \nomj \forall \cnomm \, (\wdia \nomj \leq \cnomm \Rarr \wdia \wdia \nomj \leq \cnomm)$
\end{center}

\noindent which can be written as a structural rule in the language of display calculi as follows:

\begin{center}
\AXC{$\WDIA X \vd Y$}
\LL{\fns $4$}
\UIC{$\WDIA \WDIA X \vd Y$}
\DP
\end{center}

We now provide a derivation of the axiom $(4)$ in the basic display calculus $\mathbf{D.L}$ expanded with the previous structural rule $4$.

{\small
\begin{center}
\AXC{ \ }
\LL{\fns Id$_A$}
\UIC{$A \vd A$}
\RL{\fns $\wdia_R$}
\UIC{$\WDIA A \vd \wdia A$}
\LL{\fns $4$}
\UIC{$\WDIA \WDIA A \vd \wdia A$}
\RL{\fns $\wdia \dashv \bbox$}
\UIC{$\WDIA A \vd \BBOX \wdia A$}
\LL{\fns $\wdia_L$}
\UIC{$\wdia A \vd \BBOX \wdia A$}
\LL{\fns $\wdia \dashv \bbox^{-1}$}
\UIC{$\WDIA \wdia A \vd \wdia A$}
\LL{\fns $\wdia_L$}
\UIC{$\wdia \wdia A \vd \wdia A$}
\DP
\end{center}
 }

Further processing the axiom $(4)$ using ALBA we obtain the equivalent first order correspondent (in the so-called `flat form'):

\begin{center}
$\forall \nomj \forall \nomh \forall \cnomm \, (\wdia \nomj \leq \cnomm \Rarr (\nomh \leq \wdia \nomj \Rarr \wdia \nomh \leq \cnomm))$
\end{center}

\noindent which can be written as a structural rule in the language of ALBA labelled calculi as follows:

\begin{center}
\AXC{$\Gamma \vd \wdia \nomj \leq \cnomm, \Delta$}
\LL{\fns $4$}
\UIC{$\Gamma, \nomh \leq \wdia \nomj \vd \wdia \nomh \leq \cnomm, \Delta$}
\DP
\end{center}

We now provide a derivation of the axiom $(4)$ in the basic labelled calculus $\mathbf{A.L}$ expanded with the previous structural rule $4$.

{\small 
\begin{center}
\AXC{ \ }
\LL{\fns Id$_A$}
\UIC{$\nomj \leq A \vd \nomj \leq A$}
\RL{\fns $\wdia_S$}
\UIC{$\wdia A \leq \cnomm, \nomj \leq A, \vd \wdia \nomj \leq \cnomm$}
\LL{\fns $4$}
\UIC{$\wdia A \leq \cnomm, \nomj \leq A, \nomh \leq \wdia \nomj \vd \wdia \nomh \leq \cnomm$}
\RL{\fns $\wdia \dashv \bbox$}
\UIC{$\wdia A \leq \cnomm, \nomj \leq A, \nomh \leq \wdia \nomj \vd \nomh \leq \bbox \cnomm$}
\RL{\fns S}
\UIC{$\wdia A \leq \cnomm, \bbox \cnomm \leq  \cnomm', \nomj \leq A \vd \wdia \nomj \leq \cnomm'$}
\LL{\fns $\wdia_P$}
\UIC{$\wdia A \leq \cnomm, \bbox \cnomm \leq  \cnomm' \vd \wdia A \leq \cnomm'$}
\RL{\fns S}
\UIC{$\wdia A \leq \cnomm, \nomj' \leq \wdia A \vd \nomj' \leq \bbox \cnomm$}
\LL{\fns $\wdia \dashv \bbox^{-1}$}
\UIC{$\wdia A \leq \cnomm, \nomj' \leq \wdia A \vd \wdia \nomj' \leq \cnomm$}
\LL{\fns $\wdia_P$}
\UIC{$\wdia A \leq \cnomm \vd \wdia \wdia A \leq \cnomm$}
\DP
\end{center}
 }

\paragraph{\textbf{Reflexivity.}}

Let us consider the axiom (T)\  $\wbox A \vdash A$. Using ALBA we generate the first order correspondent:

\begin{center}
$\forall \nomj \forall \cnomm \, (\nomj \leq \wbox \cnomm \Rarr \nomj \leq \cnomm)$
\end{center}

\noindent which can be written as a structural rule in the language of display calculi as follows:

\begin{center}
\AXC{$X \vd \WBOX Y$}
\RL{\fns $T$}
\UIC{$X \vd Y$}
\DP
\end{center}

We now provide a derivation of the axiom $(T)$ in the basic display calculus $\mathbf{D.L}$ expanded with the previous structural rule $T$.

{\small
\begin{center}
\AXC{ \ }
\LL{\fns Id$_A$}
\UIC{$A \vd A$}
\RL{\fns $\wbox_L$}
\UIC{$\wbox A \vd \WBOX A$}
\RL{\fns $T$}
\UIC{$\wbox A \vd A$}
\DP
\end{center}
 }

The first order correspondent of axiom (T) generated using ALBA is already in the so-called `flat form', therefore it can be written as a structural rule in the language of algebraic labelled calculi as follows:

\begin{center}
\AXC{$\Gamma \vd \nomj \leq \wbox \cnomm, \Delta$}
\RL{\fns $T$}
\UIC{$\Gamma \vd \nomj \leq \cnomm, \Delta$}
\DP
\end{center}

We now provide a derivation of the axiom (T) in the basic labelled calculus $\mathbf{A.L}$ expanded with the previous structural rule $T$.

{\small 
\begin{center}
\AXC{ \ }
\LL{\fns Id$_A$}
\UIC{$ A \leq \cnomm \vd A \leq \cnomm$}
\RL{\fns $\wbox_P$}
\UIC{$\nomj \leq \wbox A, A \leq \cnomm \vd \nomj \leq \wbox \cnomm$}
\RL{\fns $T$}
\UIC{$\nomj \leq \wbox A, A \leq \cnomm \vd \nomj \leq \cnomm$}
\RL{\fns $S$}
\UIC{$\nomj \leq \wbox A \vd \nomj \leq A$}
\DP
\end{center}
 }

\paragraph{\textbf{Symmetry.}}

Let us consider the axiom (B)\  $A \vdash \wbox \wdia A$. Using ALBA we generate the first order correspondent:

\begin{center}
$\forall \nomj  \forall \cnomm \, (\wdia \nomj\leq  \cnomm\Rarr  \nomj\leq \wbox \cnomm)$
\end{center}

\noindent which can be written as a structural rule in the language of display calculi as follows:

\begin{center}
\AXC{$\WDIA X \vd Y$}
\RL{\fns $B$}
\UIC{$X \vd \WBOX Y$}
\DP
\end{center}

We now provide a derivation of the axiom (B) in the basic display calculus $\mathbf{D.L}$ expanded with the previous structural rule $B$.

{\small
\begin{center}
\AXC{ \ }
\LL{\fns Id$_A$}
\UIC{$A \vd A$}
\RL{\fns $\wbox_R$}
\UIC{$\WDIA A \vd \wdia A$}
\RL{\fns $B$}
\UIC{$A \vd \WBOX \wdia A$}
\RL{\fns $\wbox_R$}
\UIC{$A \vd \wbox \wdia A$}
\DP
\end{center}
 }

The first order correspondent of axiom (B) generated using ALBA is already in the so-called `flat form', therefore it can be written as a structural rule in the language of algebraic labelled calculi as follows:

\begin{center}
\AXC{$\Gamma \vd \wdia \nomj\leq \cnomm, \Delta$}
\RL{\fns $B$}
\UIC{$\Gamma \vd \nomj\leq \wbox \cnomm, \Delta$}
\DP
\end{center}

We now provide a derivation of the axiom (B) in the basic labelled calculus $\mathbf{A.L}$ expanded with the previous structural rule $B$.

{\small
\begin{center}
\AXC{ \ }
\RL{\fns Id$_A$}
\UIC{$\nomj \leq A \vd \nomj \leq A$}
\RL{\fns $\wdia_S$}
\UIC{$\wdia A \leq \cnomm, \nomj \leq A \vd \wdia \nomj \leq \cnomm$}
\LL{\fns $B$}
\UIC{$\wdia A \leq \cnomm, \nomj \leq A \vd \nomj \leq \wbox \cnomm$}
\LL{\fns $\wbox_S$}
\UIC{$\nomj \leq A \vd \nomj \leq \wbox \wdia A$}
\DP
\end{center}
 }
 
\paragraph{\textbf{Co-symmetry. }}

Let us consider the axiom (B$^{-1}$)\  $\wdia \wbox A \vdash A$. Using ALBA we generate the first order correspondent:

\begin{center}
$\forall \nomj  \forall \cnomm \, (\nomj\leq \wbox \cnomm \Rarr  \wdia\nomj\leq \cnomm)$ 
\end{center}

\noindent which can be written as a structural rule in the language of display calculi as follows:

\begin{center}
\AXC{$X \vd \WBOX Y$}
\LL{\fns $B^{-1}$}
\UIC{$\WDIA X \vd Y$}
\DP
\end{center}

We now provide a derivation of the axiom (B$^{-1}$) in the basic display calculus $\mathbf{D.L}$ expanded with the previous structural rule $B^{-1}$.

{\small
\begin{center}
\AXC{ \ }
\LL{\fns Id$_A$}
\UIC{$A \vd A$}
\LL{\fns $\wbox_L$}
\UIC{$\wbox A \vd \WBOX A$}
\LL{\fns $B^{-1}$}
\UIC{$\WDIA \wbox A \vd A$}
\LL{\fns $\wdia_L$}
\UIC{$\wdia \wbox A \vd A$}
\DP
\end{center}
 }

The first order correspondent of axiom (B$^{-1}$) generated using ALBA is already in the so-called `flat form', therefore it can be written as a structural rule in the language of algebraic labelled calculi as follows:

\begin{center}
\AXC{$\Gamma \vd \nomj\leq \wbox \cnomm, \Delta$}
\LL{\fns $B^{-1}$}
\UIC{$\Gamma \vd \wdia\nomj\leq \cnomm, \Delta$}
\DP
\end{center}

We now provide a derivation of the axiom (B$^{-1}$) in the basic labelled calculus $\mathbf{A.L}$ expanded with the previous structural rule $B^{-1}$.

{\small
\begin{center}
\AXC{ \ }
\RL{\fns Id$_A$}
\UIC{$A \leq \cnomm \vd A \leq \cnomm $}
\LL{\fns $\wbox_P$}
\UIC{$\nomj \leq \wbox A, A \leq \cnomm \vd \nomj \leq \wbox \cnomm$}
\LL{\fns $B^{-1}$}
\UIC{$\nomj \leq \wbox A, A \leq \cnomm \vd \wdia \nomj \leq \cnomm$}
\LL{\fns $\wdia_L$}
\UIC{$A \leq \cnomm \vd \wdia \wbox A \cnomm$}
\DP
\end{center}
 }

\paragraph{\textbf{Confluence.}}

Let us consider the axiom (C)\  $\wdia \wbox A \vdash \wbox \wdia A$. Using ALBA we generate the first order correspondent:

\begin{center}
$\forall \nomj  \forall \cnomm \, (\wdia \bdia\nomj\leq \cnomm\Rarr  \bdia\wdia\nomj\leq \cnomm)$
\end{center}

\noindent which can be written as a structural rule in the language of display calculi as follows:

\begin{center}
\AXC{$\WDIA \BDIA X \vd Y$}
\LL{\fns $C$}
\UIC{$\BDIA \WDIA X \vd Y$}
\DP
\end{center}

We now provide a derivation of the axiom (C) in the basic display calculus $\mathbf{D.L}$ expanded with the previous structural rule $C$.

{\small
\begin{center}
\AXC{ \ }
\LL{\fns Id$_A$}
\UIC{$A \vd A$}
\LL{\fns $\wbox_L$}
\UIC{$\wbox A \vd \WBOX A$}
\LL{\fns $\bdia \dashv \wbox$}
\UIC{$\BDIA \wbox A \vd A$}
\RL{\fns $\wdia_R$}
\UIC{$\WDIA \BDIA \wbox A \vd \wdia A$}
\LL{\fns $C$}
\UIC{$\BDIA \WDIA \wbox A \vd \wdia A$}
\RL{\fns $\bdia \dashv \wbox^{-1}$}
\UIC{$\WDIA \wbox A \vd \WBOX \wdia A$}
\LL{\fns $\wdia_L$}
\UIC{$\wdia \wbox A \vd \WBOX \wdia A$}
\RL{\fns $\wbox_R$}
\UIC{$\wdia \wbox A \vd \wbox \wdia A$}
\DP
\end{center}
 }

Further processing the axiom (C) using ALBA we obtain the equivalent first order correspondent (in the so-called `flat form'):

\begin{center}
$\forall \nomj  \forall \cnomm \forall \nomh\exists \nomk\, ((\nomk\leq  \bdia\nomj\Rarr \wdia \nomk\leq \cnomm)\Rarr (\nomh\leq \wdia\nomj\Rarr \bdia\nomh\leq \cnomm))$
\end{center}

\noindent which can be written as a structural rule in the language of ALBA labelled calculi as follows, where $\nomk$ is an eigenvariable:

\begin{center}
\AXC{$\Gamma, \nomk\leq \bdia\nomj \vd \wdia \nomk\leq \cnomm, \Delta$}
\LL{\fns $C$}
\UIC{$\Gamma, \nomh\leq \wdia\nomj \vd \bdia\nomh\leq \cnomm, \Delta$}
\DP
\end{center}
